Incentive Design and Utility Learning via Energy Disaggregation

The utility company has many motivations for modifying energy consumption patterns of consumers such as revenue decoupling and demand response programs. We model the utility company--consumer interaction as a principal--agent problem. We present an iterative algorithm for designing incentives while estimating the consumer's utility function. Incentives are designed using the aggregated as well as the disaggregated (device level) consumption data. We simulate the iterative control (incentive design) and estimation (utility learning and disaggregation) process for examples including the design of incentives based on the aggregate consumption data as well as the disaggregated consumption data.

==> makefile <==
# set latexfile to the name of the main file without the .tex
latexfile = 2014Arxiv
# put the names of figure files here.  include the .eps
#figures = 
# if no references, run "touch latexfile.bbl; touch referencefile.bib"
# or delete dependency in .dvi and tarball sections
referencefile = 2014Arxiv

TEX = pdflatex

# support subdirectories
VPATH = Figs

# reruns latex if needed.  to get rid of this capability, delete the
# three lines after the rule.  Delete .bbl dependency if not using
# BibTeX references.
# idea from http://ctan.unsw.edu.au/help/uk-tex-faq/Makefile
$(latexfile).pdf : $(figures) $(latexfile).tex 
#$(latexfile).dvi : $(figures) $(latexfile).tex $(latexfile).bbl
	while ($(TEX) $(latexfile) ; \
	grep -q "Rerun to get cross" $(latexfile).log ) do true ; \
	done


# keep .eps files in the same directory as the .fig files
#%.eps : %.fig
#	fig2dev -L eps $< > $(dir $< )$@

#$(latexfile).pdf : $(latexfile).ps
#	ps2pdf $(latexfile).ps $(latexfile).pdf

#pdf : $(latexfile).pdf

#$(latexfile).ps : $(latexfile).dvi
#	dvips $(latexfile)

#ps : $(latexfile).ps 

# make can't know all the sourcefiles.  some file may not have
# sourcefiles, e.g. eps's taken from other documents. 
$(latexfile).tar.gz : $(figures) $(latexfile).tex $(referencefile).bib
	tar -czvf $(latexfile).tar.gz $^

tarball: $(latexfile).tar.gz

cpall:
	make; skim $(latexfile).pdf

clean:
	rm $(latexfile).dvi $(latexfile).log $(latexfile).ps $(latexfile).pdf

